Image Captioners Are Scalable Vision Learners Too

Contrastive pretraining on image-text pairs from the web is one of the most popular large-scale pretraining strategies for vision backbones, especially in the context of large multimodal models. At the same time, image captioning on this type of data is commonly considered an inferior pretraining strategy. In this paper, we perform a fair comparison of these two pretraining strategies, carefully matching training data, compute, and model capacity. Using a standard encoder-decoder transformer, we find that captioning alone is surprisingly effective: on classification tasks, captioning produces vision encoders competitive with contrastively pretrained encoders, while surpassing them on vision & language tasks. We further analyze the effect of the model architecture and scale, as well as the pretraining data on the representation quality, and find that captioning exhibits the same or better scaling behavior along these axes. Overall our results show that plain image captioning is a more powerful pretraining strategy than was previously believed.

==> tbls/deprecated_10shot_9b.tex <==
\begin{table}[]
\caption{10shot linear evaluation accuracy on the pre-logit representation. \genp outperfroms \gen and achives overall comparable results with \clip trained with a batch size of 16k.}
\label{tbl:results:10shot_main_9b}
\footnotesize
    \centering

\begin{tabular}{lrrrrr}
\toprule
& imagenet & cifar100 & pets & cars\\
  \midrule
Cap & 57.2{\tiny$\pm$0.1} & 58.6{\tiny$\pm$0.8} & 83.7{\tiny$\pm$0.6} & 84.2{\tiny$\pm$0.1} \\
CapPa & \textbf{59.1{\tiny$\pm$0.1}} & 62.4{\tiny$\pm$0.4} & \textbf{86.5{\tiny$\pm$0.1}} & \textbf{86.6{\tiny$\pm$0.2}} \\
CLIP* (8k) & 58.5{\tiny$\pm$0.1} & 64.9{\tiny$\pm$0.4} & 77.7{\tiny$\pm$1.5} & 80.8{\tiny$\pm$0.4} \\
CLIP* (16k) & \textbf{59.7{\tiny$\pm$0.4}} & \textbf{66.3{\tiny$\pm$0.2}} & 80.6{\tiny$\pm$1.2} & 82.9{\tiny$\pm$0.1} \\
\textcolor{gray}{CLIP} & \textcolor{gray}{59.0{\tiny$\pm$0.2}} & \textcolor{gray}{68.6{\tiny$\pm$0.1}} & \textcolor{gray}{82.1{\tiny$\pm$0.7}} & \textcolor{gray}{70.2{\tiny$\pm$0.7}} \\
  \midrule
CapPa L/14 & \textbf{70.6{\tiny$\pm$0.2}} & \textbf{72.9{\tiny$\pm$0.4}} & \textbf{92.6{\tiny$\pm$0.5}} & \textbf{92.2{\tiny$\pm$0.2}} \\
CLIP* L/14 & 69.8{\tiny$\pm$0.1} & \textbf{74.1{\tiny$\pm$0.5}} & 87.7{\tiny$\pm$0.9} & 89.2{\tiny$\pm$0.2} \\
\textcolor{gray}{CLIP L/14} & \textcolor{gray}{69.7{\tiny$\pm$0.1}} & \textcolor{gray}{79.4{\tiny$\pm$0.3}} & \textcolor{gray}{90.4{\tiny$\pm$0.8}} & \textcolor{gray}{81.1{\tiny$\pm$0.4}} \\
\bottomrule
\end{tabular}
\end{table}



==> tbls/deprecated_aro.tex <==
\begin{table}[]
\caption{Results on the Attribute, Relation and Order (ARO) benchmark \cite{aro}. \gen and \genp models clearly outperform all \clip and \oaiclip variants across all data sets. They also outperform NegCLIP \cite{aro} which was explicitly trained to be sensitive to word ordering and attribution.}
\label{tbl:results:aro_eval}
\setlength{\tabcolsep}{3pt}
\footnotesize
    \centering
\begin{tabular}{lcccc}
\toprule
{}  & Attrib. &  VG Rel. &  Order (F) &  Order (C) \\
\midrule
No img    &  83.7 &   86.2 &   98.8 &  98.7 \\
\gen           & 88.9 &  86.6 &  99.1 & 99.0 \\
\genp           & 85.7 &  86.7 &   99.2 &  98.8 \\ 
% PlaCaP      & L/14 & 89.3 &  86.0 &   99.3 &   99.0 \\ \midrule
% CLIP* (8k)       & B/16 & 55.4 &  39.8 &  43.7 & 32.8 \\
\clip      &  53.2 &  39.7 &  45.5 & 37.0 \\ \midrule
% CLIP* (16k) & L/14 & 57.8 & 35.9 &    40.2 & 31.5 \\ \midrule
% CLIP             & B/32 & 63.2 &  59.1 &  59.4 &  47.3 \\
\oaiclip             &  62.7 &  58.7 &  57.9 &  49.5\\
ARO Best &  73.0 & 88.0 & 60.0 & 46.0 \\
NegCLIP             &   71.0 &   81.0 &  91.0 &  86.0 \\
\bottomrule
\end{tabular}
\end{table}



==> tbls/deprecated_lit_transfer.tex <==
\begin{table*}[t]
\footnotesize
  \setlength{\tabcolsep}{0pt}
  \setlength{\extrarowheight}{5pt}
  \renewcommand{\arraystretch}{0.75}
  \newcolumntype{C}{>{\centering\arraybackslash}X}
  \newcolumntype{R}{>{\raggedleft\arraybackslash}X}
  \centering
  \caption{\mt{nit: Gray out original CLIP}
    Frozen transfer for zero-shot classification and retrieval via LiT~\cite{lit}. Especially for the larger model, CapPa is competitve with CLIP with comparable or fewer examples seen.
  }\label{tbl:results:lit}
  % Format is type{width}, p: paragraph, top-align, C is custom, c is squeezed.

  \begin{tabularx}{0.5\linewidth}{p{1.5cm}p{0.2cm}Cp{0.01cm}Cp{0.2cm}Cp{0.01cm}Cp{0.2cm}Cp{0.01cm}C}
    \toprule[1pt]
 && \multicolumn{3}{c}{INet 0shot} && \multicolumn{3}{c}{COCO t2i} && \multicolumn{3}{c}{COCO i2t} \\ 
\cmidrule[0.5pt]{3-5} \cmidrule[0.5pt]{7-9} \cmidrule[0.5pt]{11-13}
LiT pairs: && 3B && 12B && 3B && 12B && 3B && 12B \\ 
    \midrule
Cap && 67.8 && 69.0 && 37.5 && 39.1 && 53.9 && 54.8 \\ 
CapPa && 68.8 && \textbf{70.2} && 37.3 && 38.6 && 53.9 && 55.1 \\ 
CLIP* && 69.0 && 70.0 && 38.9 && \textbf{40.1} && 55.1 && \textbf{57.0} \\ 
CLIP~\cite{clip} && \multicolumn{3}{c}{68.3} && \multicolumn{3}{c}{32.3} && \multicolumn{3}{c}{52.8} \\ 
\midrule
CapPa L/14 && 76.4 && \textbf{77.5} && 43.9 && 45.4 && 60.3 && \textbf{62.6} \\ 
CLIP* L/14 && 75.8 && 76.6 && 44.7 && \textbf{46.3} && 60.7 && 62.3 \\ 
CLIP L/14 && \multicolumn{3}{c}{75.1} && \multicolumn{3}{c}{36.5} && \multicolumn{3}{c}{56.6} \\ 


  \bottomrule
  \end{tabularx}
\end{table*}


==> tbls/deprecated_lit_transfer_old.tex <==
\begin{table*}[t]
\footnotesize
  \setlength{\tabcolsep}{0pt}
  \setlength{\extrarowheight}{5pt}
  \renewcommand{\arraystretch}{0.75}
  \newcolumntype{C}{>{\centering\arraybackslash}X}
  \newcolumntype{R}{>{\raggedleft\arraybackslash}X}
  \centering
  \caption{
    Frozen LiT 0shot classification transfer and retrieval. The main take-away is that in terms of \emph{linear} transfer, CLIP seems clearly better. However, re-learning the ``summarization'' of tokens into a single feature vector (via MAP head) mostly eliminates the difference in performance.\lb{describe better.}
  }\label{tbl:results:lit}
  % Format is type{width}, p: paragraph, top-align, C is custom, c is squeezed.
  \begin{tabularx}{0.75\linewidth}{p{2.0cm}p{0.01cm}Cp{0.01cm}Cp{0.01cm}Cp{0.01cm}Cp{0.01cm}Cp{0.01cm}C}
    \toprule[1pt]
Pretraining && GAP (i1k) && MAP (i1k) && GAP (t2i) && MAP (t2i) && GAP (i2t) && MAP (i2t) \\ 
    \midrule
\gen && 62.1 && 65.9 && 30.6 && 35.3 && 46.8 && 50.3 \\ 
\genp && 62.2 && 66.4 && 29.4 && 34.3 && 46.8 && 49.7 \\ 
\clip (8k) && 66.0 && 65.9 && 35.8 && 36.5 && 52.6 && 52.0 \\ 
\clip (16k) && 67.2 && 66.7 && 36.1 && 37.0 && 53.6 && 53.0 \\ 

  \bottomrule
  \end{tabularx}
\end{table*}

==> tbls/sugarcrepe_examples_inline.tex <==
\begin{table}
\footnotesize
  \setlength{\tabcolsep}{0pt}
  \setlength{\extrarowheight}{5pt}
  \renewcommand{\arraystretch}{0.75}
  \newcolumntype{L}{>{\raggedright\arraybackslash}X}
  \centering
  \caption{
    Representative examples of CapPa L/14 wins (first three) and losses (fourth) over CLIP L/14 on the different {\bf replace} categories of the SugarCrepe hard negatives benchmark suite.
    See text for example selection criteria.
    Higher score means better: for CapPa this is the log-likelihood, so closer to 0 is better, while for CLIP this is the matching score (multiplied by 100) so closer to 100 is better.
  }\label{tbl:results:sc_examples_repl}
\begin{tabularx}{\linewidth}{p{0.3cm}p{0.1cm}p{0.3cm}p{0.1cm}Lp{0.15cm}Lp{0.15cm}Lp{0.15cm}L}
  \toprule[1pt]
 && && \multicolumn{5}{c}{\bf CapPa wins over CLIP} && \multicolumn{1}{c}{\bf CLIP wins over CapPa} \\
  \cmidrule[0.5pt]{5-9} \cmidrule[0.5pt]{11-11}
\multirow{5}{*}{\rotatebox{90}{\hspace*{-0.7cm}\textbf{Replace Object}}}
 && \multirow{2}{*}{\rotatebox{90}{\hspace*{-0.7cm}Positive}}
 && CapPa:\textbf{-28.6} CLIP:\textbf{23.6}
 && CapPa:\textbf{-45.4} CLIP:\textbf{13.2}
 && CapPa:\textbf{-42.4} CLIP:\textbf{16.8}
 && CapPa:\textbf{-54.6} CLIP:\textbf{13.7}
 \\ &&
 && \textit{Street signs on the corner of Gladys and Detroit}
 && \textit{A run down building with two planters outside the door}
 && \textit{A brown bird has a small yellow head.}
 && \textit{The model toys are positioned on the table.}
 \\ && \multirow{2}{*}{\rotatebox{90}{\hspace*{-0.7cm}Negative}}
 && CapPa:\textbf{-53.8} CLIP:\textbf{13.9}
 && CapPa:\textbf{-59.2} CLIP:\textbf{14.8}
 && CapPa:\textbf{-46.2} CLIP:\textbf{18.1}
 && CapPa:\textbf{-51.7} CLIP:\textbf{8.8}
 \\ &&
 && \textit{Street signs on the corner of Gladys and Chicago.}
 && \textit{A run down building with a statue outside the door.}
 && \textit{A brown bird has a small yellow beak.}
 && \textit{The books are positioned on the table.}
 \\ &&
 && \vspace{0pt}\centerline{\includegraphics[width=3cm,height=3cm,keepaspectratio]{figs/cocoval/COCO_val2014_000000058636.jpg}}
 && \vspace{0pt}\centerline{\includegraphics[width=3cm,height=3cm,keepaspectratio]{figs/cocoval/COCO_val2014_000000502136.jpg}}
 && \vspace{0pt}\centerline{\includegraphics[width=3cm,height=3cm,keepaspectratio]{figs/cocoval/COCO_val2014_000000561009.jpg}}
 && \vspace{0pt}\centerline{\includegraphics[width=3cm,height=3cm,keepaspectratio]{figs/cocoval/COCO_val2014_000000429011.jpg}}
 \\
\midrule
\multirow{5}{*}{\rotatebox{90}{\hspace*{-0.7cm}\textbf{Replace Attribute}}}
 && \multirow{2}{*}{\rotatebox{90}{\hspace*{-0.7cm}Positive}}
 && CapPa:\textbf{-45.0} CLIP:\textbf{14.7}
 && CapPa:\textbf{-47.3} CLIP:\textbf{13.1}
 && CapPa:\textbf{-17.3} CLIP:\textbf{15.7}
 && CapPa:\textbf{-115.9} CLIP:\textbf{14.1}
 \\ &&
 && \textit{A plate of food with a fried egg and colorful vegetables.}
 && \textit{A bunch of different foods on display on  a counter.}
 && \textit{A large black truck in a parking lot.}
 && \textit{Two large trucks are travelling along a tree-lined roadway.}
 \\ && \multirow{2}{*}{\rotatebox{90}{\hspace*{-0.7cm}Negative}}
 && CapPa:\textbf{-59.5} CLIP:\textbf{15.1}
 && CapPa:\textbf{-53.8} CLIP:\textbf{14.8}
 && CapPa:\textbf{-38.3} CLIP:\textbf{16.1}
 && CapPa:\textbf{-61.7} CLIP:\textbf{12.5}
 \\ &&
 && \textit{A plate of food with a fried egg and monochromatic vegetables.}
 && \textit{A bunch of similar foods on display on a counter.}
 && \textit{A small black truck in a parking lot.}
 && \textit{Two large trucks are travelling along a deserted roadway.}
 \\ &&
 && \vspace{0pt}\centerline{\includegraphics[width=3cm,height=3cm,keepaspectratio]{figs/cocoval/COCO_val2014_000000533958.jpg}}
 && \vspace{0pt}\centerline{\includegraphics[width=3cm,height=3cm,keepaspectratio]{figs/cocoval/COCO_val2014_000000226903.jpg}}
 && \vspace{0pt}\centerline{\includegraphics[width=3cm,height=3cm,keepaspectratio]{figs/cocoval/COCO_val2014_000000123131.jpg}}
 && \vspace{0pt}\centerline{\includegraphics[width=3cm,height=3cm,keepaspectratio]{figs/cocoval/COCO_val2014_000000569565.jpg}}
 \\
\midrule
\multirow{5}{*}{\rotatebox{90}{\hspace*{-0.7cm}\textbf{Replace Relation}}}
 && \multirow{2}{*}{\rotatebox{90}{\hspace*{-0.7cm}Positive}}
 && CapPa:\textbf{-20.0} CLIP:\textbf{18.5}
 && CapPa:\textbf{-48.2} CLIP:\textbf{18.6}
 && CapPa:\textbf{-29.1} CLIP:\textbf{24.4}
 && CapPa:\textbf{-55.6} CLIP:\textbf{17.6}
 \\ &&
 && \textit{A fire hydrant in a grassy field next to a bush}
 && \textit{A cell phone on top of a calculator near a computer keyboard.}
 && \textit{A red fire hydrant on a city sidewalk.}
 && \textit{A train driving over a small bridge on a green hillside.}
 \\ && \multirow{2}{*}{\rotatebox{90}{\hspace*{-0.7cm}Negative}}
 && CapPa:\textbf{-56.1} CLIP:\textbf{21.5}
 && CapPa:\textbf{-56.1} CLIP:\textbf{19.2}
 && CapPa:\textbf{-35.6} CLIP:\textbf{25.6}
 && CapPa:\textbf{-54.7} CLIP:\textbf{17.4}
 \\ &&
 && \textit{A fire hydrant in a grassy field far from a bush.}
 && \textit{A cell phone underneath a calculator near a computer keyboard.}
 && \textit{A red fire hydrant beside a city sidewalk.}
 && \textit{A train passing under a small bridge on a green hillside.}
 \\ &&
 && \vspace{0pt}\centerline{\includegraphics[width=3cm,height=3cm,keepaspectratio]{figs/cocoval/COCO_val2014_000000087875.jpg}}
 && \vspace{0pt}\centerline{\includegraphics[width=3cm,height=3cm,keepaspectratio]{figs/cocoval/COCO_val2014_000000561366.jpg}}
 && \vspace{0pt}\centerline{\includegraphics[width=3cm,height=3cm,keepaspectratio]{figs/cocoval/COCO_val2014_000000038048.jpg}}
 && \vspace{0pt}\centerline{\includegraphics[width=3cm,height=3cm,keepaspectratio]{figs/cocoval/COCO_val2014_000000579818.jpg}}
 \\
 \bottomrule
  \end{tabularx}
\end{table}

\begin{table}
\footnotesize
  \setlength{\tabcolsep}{0pt}
  \setlength{\extrarowheight}{5pt}
  \renewcommand{\arraystretch}{0.75}
  \newcolumntype{L}{>{\raggedright\arraybackslash}X}
  \centering
  \caption{
    Representative examples of CapPa L/14 wins (first three) and losses (fourth) over CLIP L/14 on the different {\bf add} categories of the SugarCrepe hard negatives benchmark suite.
    See text for example selection criteria.
    Higher score means better: for CapPa this is the log-likelihood, so closer to 0 is better, while for CLIP this is the matching score (multiplied by 100) so closer to 100 is better.
  }\label{tbl:results:sc_examples_add}
\begin{tabularx}{\linewidth}{p{0.3cm}p{0.1cm}p{0.3cm}p{0.1cm}Lp{0.15cm}Lp{0.15cm}Lp{0.15cm}L}
  \toprule[1pt]
 && && \multicolumn{5}{c}{\bf CapPa wins over CLIP} && \multicolumn{1}{c}{\bf CLIP wins over CapPa} \\
  \cmidrule[0.5pt]{5-9} \cmidrule[0.5pt]{11-11}
\multirow{7}{*}{\rotatebox{90}{\hspace*{-0.7cm}\textbf{Add Object}}}
 && \multirow{2}{*}{\rotatebox{90}{\hspace*{-0.7cm}Positive}}
 && CapPa:\textbf{-18.2} CLIP:\textbf{13.7}
 && CapPa:\textbf{-30.2} CLIP:\textbf{14.3}
 && CapPa:\textbf{-27.3} CLIP:\textbf{14.0}
 && CapPa:\textbf{-60.3} CLIP:\textbf{22.5}
 \\ &&
 && \textit{A bathroom with a mirror and a sink.}
 && \textit{A two layered cake sits on a table top}
 && \textit{an image of a plate of food with meat and veggies}
 && \textit{A bridge and groom cutting their wedding cake that has fruit on top.}
 \\ && \multirow{2}{*}{\rotatebox{90}{\hspace*{-0.7cm}Negative}}
 && CapPa:\textbf{-150.3} CLIP:\textbf{13.7}
 && CapPa:\textbf{-64.9} CLIP:\textbf{15.5}
 && CapPa:\textbf{-148.6} CLIP:\textbf{14.6}
 && CapPa:\textbf{-53.4} CLIP:\textbf{21.6}
 \\ &&
 && \textit{A bathroom with a mirror, sink, and shower.}
 && \textit{A two layered cake sits on a table top next to a vase of flowers.}
 && \textit{An image of a plate of food with meat, fruit, and veggies.}
 && \textit{A bride and groom cutting their wedding cake that has flowers and fruit on top.}
 \\ &&
 && \vspace{0pt}\centerline{\includegraphics[width=3cm,height=3cm,keepaspectratio]{figs/cocoval/COCO_val2014_000000368940.jpg}}
 && \vspace{0pt}\centerline{\includegraphics[width=3cm,height=3cm,keepaspectratio]{figs/cocoval/COCO_val2014_000000173383.jpg}}
 && \vspace{0pt}\centerline{\includegraphics[width=3cm,height=3cm,keepaspectratio]{figs/cocoval/COCO_val2014_000000104612.jpg}}
 && \vspace{0pt}\centerline{\includegraphics[width=3cm,height=3cm,keepaspectratio]{figs/cocoval/COCO_val2014_000000276434.jpg}}
 \\  && \multirow{2}{*}{\rotatebox{90}{\hspace*{-0.7cm}Pos (fixed)}}
 && 
 && 
 && 
 && CapPa:\textbf{-46.1} CLIP:\textbf{22.7}
 \\ &&
 && \textit{}
 && \textit{}
 && \textit{}
 && \textit{A bride and groom cutting their wedding cake that has fruit on top.\vspace{0.25cm}}
 \\
\midrule
\multirow{7}{*}{\rotatebox{90}{\hspace*{-0.7cm}\textbf{Add Attribute}}}
 && \multirow{2}{*}{\rotatebox{90}{\hspace*{-0.7cm}Positive}}
 && CapPa:\textbf{-43.8} CLIP:\textbf{21.0}
 && CapPa:\textbf{-65.4} CLIP:\textbf{16.1}
 && CapPa:\textbf{-49.9} CLIP:\textbf{17.6}
 && CapPa:\textbf{-62.1} CLIP:\textbf{20.4}
 \\ &&
 && \textit{A little girl smiling for the camera with an umbrella behind her.}
 && \textit{A clock fastened to a brick store front reads 10 after 10}
 && \textit{A person frying some kind of food on a stove.}
 && \textit{There is a stuffed animal sitting on the toliet.}
 \\ && \multirow{2}{*}{\rotatebox{90}{\hspace*{-0.7cm}Negative}}
 && CapPa:\textbf{-121.5} CLIP:\textbf{21.0}
 && CapPa:\textbf{-90.7} CLIP:\textbf{17.0}
 && CapPa:\textbf{-115.3} CLIP:\textbf{19.5}
 && CapPa:\textbf{-49.8} CLIP:\textbf{19.1}
 \\ &&
 && \textit{A little girl smiling for the camera with a polka-dotted umbrella behind her.}
 && \textit{A clock fastened to a lush brick store front reads 10 after 10.}
 && \textit{A person frying some curry-spiced food on a stove.}
 && \textit{There is a stuffed animal sitting on the decorated toilet.}
 \\ &&
 && \vspace{0pt}\centerline{\includegraphics[width=3cm,height=3cm,keepaspectratio]{figs/cocoval/COCO_val2014_000000466125.jpg}}
 && \vspace{0pt}\centerline{\includegraphics[width=3cm,height=3cm,keepaspectratio]{figs/cocoval/COCO_val2014_000000488736.jpg}}
 && \vspace{0pt}\centerline{\includegraphics[width=3cm,height=3cm,keepaspectratio]{figs/cocoval/COCO_val2014_000000580294.jpg}}
 && \vspace{0pt}\centerline{\includegraphics[width=3cm,height=3cm,keepaspectratio]{figs/cocoval/COCO_val2014_000000376442.jpg}}
 \\  && \multirow{2}{*}{\rotatebox{90}{\hspace*{-0.7cm}Pos (fixed)}}
 && 
 && 
 && 
 && CapPa:\textbf{-36.8} CLIP:\textbf{21.3}
 \\ &&
 && \textit{}
 && \textit{}
 && \textit{}
 && \textit{There is a stuffed animal sitting on the toilet.\vspace{0.25cm}}
 \\
 \bottomrule
  \end{tabularx}
\end{table}

\begin{table}
\footnotesize
  \setlength{\tabcolsep}{0pt}
  \setlength{\extrarowheight}{5pt}
  \renewcommand{\arraystretch}{0.75}
  \newcolumntype{L}{>{\raggedright\arraybackslash}X}
  \centering
  \caption{
    Representative examples of CapPa L/14 wins (first three) and losses (fourth) over CLIP L/14 on the different {\bf swap} categories of the SugarCrepe hard negatives benchmark suite.
    See text for example selection criteria.
    Higher score means better: for CapPa this is the log-likelihood, so closer to 0 is better, while for CLIP this is the matching score (multiplied by 100) so closer to 100 is better.
  }\label{tbl:results:sc_examples_swap}
\begin{tabularx}{\linewidth}{p{0.3cm}p{0.1cm}p{0.3cm}p{0.1cm}Lp{0.15cm}Lp{0.15cm}Lp{0.15cm}L}
  \toprule[1pt]
 && && \multicolumn{5}{c}{\bf CapPa wins over CLIP} && \multicolumn{1}{c}{\bf CLIP wins over CapPa} \\
  \cmidrule[0.5pt]{5-9} \cmidrule[0.5pt]{11-11}
\multirow{5}{*}{\rotatebox{90}{\hspace*{-0.7cm}\textbf{Swap Object}}}
 && \multirow{2}{*}{\rotatebox{90}{\hspace*{-0.7cm}Positive}}
 && CapPa:\textbf{-33.5} CLIP:\textbf{22.5}
 && CapPa:\textbf{-54.9} CLIP:\textbf{22.1}
 && CapPa:\textbf{-38.1} CLIP:\textbf{15.6}
 && CapPa:\textbf{-111.4} CLIP:\textbf{20.5}
 \\ &&
 && \textit{a bright kitchen with tulips on the table and plants by the window}
 && \textit{A person cutting a pizza next to a salad and bottles of wine on wooden table.}
 && \textit{A close up of a sandwich with a drink in the back.}
 && \textit{Statues on the second floor of a building, sitting below a clock.}
 \\ && \multirow{2}{*}{\rotatebox{90}{\hspace*{-0.7cm}Negative}}
 && CapPa:\textbf{-56.8} CLIP:\textbf{22.8}
 && CapPa:\textbf{-57.5} CLIP:\textbf{22.5}
 && CapPa:\textbf{-45.6} CLIP:\textbf{16.2}
 && CapPa:\textbf{-110.8} CLIP:\textbf{19.4}
 \\ &&
 && \textit{A bright kitchen with plants on the table and tulips by the window.}
 && \textit{A person cutting a salad next to a pizza and bottles of wine on wooden table.}
 && \textit{A close up of a drink with a sandwich in the back.}
 && \textit{A clock on the second floor of a building, sitting below statues.}
 \\ &&
 && \vspace{0pt}\centerline{\includegraphics[width=3cm,height=3cm,keepaspectratio]{figs/cocoval/COCO_val2014_000000136355.jpg}}
 && \vspace{0pt}\centerline{\includegraphics[width=3cm,height=3cm,keepaspectratio]{figs/cocoval/COCO_val2014_000000385029.jpg}}
 && \vspace{0pt}\centerline{\includegraphics[width=3cm,height=3cm,keepaspectratio]{figs/cocoval/COCO_val2014_000000120853.jpg}}
 && \vspace{0pt}\centerline{\includegraphics[width=3cm,height=3cm,keepaspectratio]{figs/cocoval/COCO_val2014_000000565989.jpg}}
 \\
\midrule
\multirow{5}{*}{\rotatebox{90}{\hspace*{-0.7cm}\textbf{Swap Attribute}}}
 && \multirow{2}{*}{\rotatebox{90}{\hspace*{-0.7cm}Positive}}
 && CapPa:\textbf{-32.6} CLIP:\textbf{15.4}
 && CapPa:\textbf{-45.9} CLIP:\textbf{19.4}
 && CapPa:\textbf{-28.4} CLIP:\textbf{16.3}
 && CapPa:\textbf{-108.6} CLIP:\textbf{19.3}
 \\ &&
 && \textit{a white cake is by a bunch of flowers}
 && \textit{A blue tennis racket has a yellow tennis ball on it.}
 && \textit{a black bike rests against a brown bed}
 && \textit{All of the cows are poking their heads out, eating some hay.}
 \\ && \multirow{2}{*}{\rotatebox{90}{\hspace*{-0.7cm}Negative}}
 && CapPa:\textbf{-64.1} CLIP:\textbf{17.3}
 && CapPa:\textbf{-54.9} CLIP:\textbf{19.5}
 && CapPa:\textbf{-52.8} CLIP:\textbf{16.9}
 && CapPa:\textbf{-107.1} CLIP:\textbf{18.2}
 \\ &&
 && \textit{A bunch of cakes are by a white flower.}
 && \textit{A yellow tennis racket has a blue tennis ball on it.}
 && \textit{a brown bike rests against a black bed.}
 && \textit{Some cows are poking their heads out, eating all of the hay.}
 \\ &&
 && \vspace{0pt}\centerline{\includegraphics[width=3cm,height=3cm,keepaspectratio]{figs/cocoval/COCO_val2014_000000556873.jpg}}
 && \vspace{0pt}\centerline{\includegraphics[width=3cm,height=3cm,keepaspectratio]{figs/cocoval/COCO_val2014_000000179285.jpg}}
 && \vspace{0pt}\centerline{\includegraphics[width=3cm,height=3cm,keepaspectratio]{figs/cocoval/COCO_val2014_000000274687.jpg}}
 && \vspace{0pt}\centerline{\includegraphics[width=3cm,height=3cm,keepaspectratio]{figs/cocoval/COCO_val2014_000000137576.jpg}}
 \\
 \bottomrule
  \end{tabularx}
\end{table}
